Proportionality in Committee Selection with Negative Feelings

We study a class of elections in which the input format is trichotomous and allows voters to elicit their negative feelings explicitly. In particular, we study multiwinner elections with a special proclivity to elect proportionally representative committees. That is, we design various axioms to deal with negative feelings and suggest some structures to these preferences that allow better preference aggregation rules. We propose two different classes of axioms designed to aggregate trichotomous preferences more efficiently. We propose trichotomous versions of some well known multiwinner voting rules and report their satisfiability of our axioms. Hence, with reports of our simulations as evidence, we build upon the social optimality of our proportionality based axioms to evaluate the quality of voting rules for electing a proportionally representative committee with trichotomous ballots as inputs.

==> ConditionalProof.tex <==
\begin{prop}
WTPSC implies Generalized Proportional Solid Coalition. 
\end{prop}
\begin{proof}
Let us assume that the committee $W$ satisfies WTPSC, which means that for all `large enough' trichotomous Solid Coalitions, there is a proportional representation in the committee. We take into account the following three cases where the set of voters which forms a solid coalition is large enough i.e. $V' \geq l\frac{n}{k}$ and the nature of the set of candidates over which the voters form the solid coalition varies.
\begin{itemize}
    \item If a set of voters $V'$ form a trichotomous solid coalition for a set of candidates $C' = C$, then every committee trivially satisfies Hare-PSC since there always exists a subset $C''$ large enough in the committee such that the candidates in it are preferred at least as much as the least preferred candidates by some voter in the solid coalition.
    \item Assume that $\forall i \in V'$ and $\forall c' \in C'$, \rutvik{to check notations in handbook of COMSOC} $c' \in max_i(V')$.\footnote{\noindent$max_i(C)$ returns the most preferred candidates from C with respect to the weak ranking of the $i^{th} $voter} So, $C' \subseteq (\cup_{i \in V'} A_i^+ \setminus \cup_{i \in V'} A_i^-)$. Since the committee satisfies WTPSC, $(\cup_{i \in V'}A_i^+) \cap W \geq l$ and since every candidate in the set $C'$ belongs to $A_i^+$ for all $i \in V'$ there always exists a subset of candidates $C'' \subseteq W$ of size $min(|C'|, l)$ such that  $\forall c'' \in C''$
    $$\exists i \in V': c'' \succeq c^{(i, |C'|)}$$
    \item Now assume that $\forall i \in V'$ and $\forall c' \in C'$, $c' \in max_{\succ_i}(C)$ or $c' \in indif_{\succ_i}(C)$\footnote{We assume that the set of solidly supported candidates does not contain those candidates which lie in the indifference class of all the voters that form the solid coalition.  } Since this set of voters does form a solid coalition, $\forall c' \in C' \text{, } \exists i \in V'\text{such that } \\
    c' \in A_i^+$\footnote{refer footnote 2}. Since every candidate in $C'$ belongs to the approval class of at least one of the voters in the solid coalition, $C' \subseteq \cup_{i \in V'}A_i+ \setminus \cup_{i \in V'}A_i^-$. Again since the committee satisfies WTPSC and additionally every candidate in $C'$ belongs to $A_i^+$ for some voter $i \in V'$, there always exists a subset of candidates $C'' \subseteq W$ of size $min(|C'|, l)$ such that $\forall c'' \in C''$ 
    $$\exists i \in V' : c'' \succeq c^{(i, |C'|)}$$
    
\end{itemize}
The only difference between the second and the third point is that in the second case, the \emph{solidly supported candidates} lie in the approval sets of each and every voter, while in the latter case, they either lie in the approval set of at least one voter. 
\end{proof}




\begin{itemize}

\item 
It makes sense to consider single-winner elections, multiwinner elections, and participatory budgeting.

\item
One thing that we can say is that adding the possibility of expressing negative feelings is, informally speaking, more ``expressive''.

To make this informal claim of some weight, we can consider the example of a voter which is OK with all the alternatives beside one; without negative feelings, he can give the cumulative vote $[1/m, \ldots, 1/m, 0]$, but the difference between $1/m$ and $0$ is very small. However, with the possibility of expressing negative feelings, such a voter can say $[0, \ldots, 0, -1]$, which is much more intense and closer to what the voter wants to express.

\item Suppose we now consider that the set of voters 
Hopefully we can show some impossibility results and, thus, formally demonstrate that there are some things that cannot be achieved without adding the possibility of expressing negative feelings.


\item
Say something about ``chores''.

\item
Some related work: ``Dilemma with approval and disapproval votes'' (and other stuff from Annick).

\end{itemize}


\nimrod{and here our paper ends, yes?}

\section{Ordinal Voting with Negative Feelings}

A natural way of adding negative feelings to ordinal elections would be to let each voter specify a ranking \textbf{and} a number between $0$ and $|A| + 1$, understood as the ``cutting point'' in the ordinal ranking, specifically such that alternatives to the left of the cutting point are to be understood as making positive feelings while alternatives to the right of the cutting point are to be understood as making negative feelings.

E.g., a vote over $A = \{a, b, c\}$ could be $a > b\ |\ c$, where $|$ means the cutting point. Then, such a vote is understood that $a$ is the best choice, then $b$, and then $c$ makes me feel negative. \\



\section{Cumulative voting with negative feelings}

A natural way of adding negative feelings to cumulative elections would be to let each voter specify a ``division of one coin'' between the alternatives \textbf{and} labeling each item with either ``positive'' or ``negative''.

Pictorially, this is like dot-voting, but where participants do not simply get stickers, but get Reversi disks.

\nimrod{Perhaps actually this is the most interesting thing that we can offer..}

\nimrod{Motivation also from the bench example}


\subsection{Single-Winner Reversi Voting}

So each voter gets $t$ Reversi disks which she can place on each of the alternatives, either as positive (say, green) or negative (say, red). Then, the \emph{score} of each alternative equals the number of green disks on it minus the number of red disks on it, and an alternative with the highest score wins.


\subsection{Multiwinner Reversi Voting}

We can use Reversi voting also for multiwinner voting by considering a $k$-best version of it:
  The \emph{score} of each alternative equals the number of green disks on it minus the number of red disks on it, and we select the $k$ top alternatives when sorted in decreasing order of their score.


\subsection{Reversi Voting for Participatory Budgeting}

We can adapt our CSTV to use Reversi voting. To see why it is important, consider the following example:
  With our CSTV we can run into the problem as follows.
  There are $3$ items, $a$, $b$, and $c$. There is budget limit $2$, and all items cost the same, that is $1$ (unit cost; so this is actually multiwinner election).
  Now, there are $5$ voters.
  For the story, say that voter $v_4$ and $v_5$ already voted, as follows:
  $v_4 : 0, 0, 1$,
  $v_5 : 0, 0, 1$.
  So, $c$ gets two points (size of stash), and $a$ and $b$ get zero.
  For the story, say that $v_1, v_2, v_3$ have very strong negative feelings towards $c$.
  Now, if we do our normal CSTV, then, even though $\{v_1, v_2, v_3\}$ is a voter majority, they cannot make it so as to not fund $c$.

However, if we use negative feelings (i.e., adapt Reversi voting here), then $v_1, v_2, v_3$ can vote as follows:
  $v_1 : 1/6, 1/6, -2/3$,
  $v_2 : 1/6, 1/6, -2/3$,
  and
  $v_3 : 1/6, 1/6, -2/3$
and get $c$ not to be funded.

==> Voting with Negative Feelings/ApprovalProportionality.tex <==

\subsection{Proportionality for Approval Ballots}

We recall two known axioms of proportional representation in approval voting for selecting a committee of size $k$.
\begin{definition}{JR \cite{JR}}
A committee $W$ is said to satisfy \emph{Justified Representation} if there does not exist group of voters $V' \subseteq V$ such that $|V'| \geq \frac{n}{k}$ and 
$(\cup_{i \in V'}A_i) \cap W = \emptyset$ 
\end{definition}
\begin{definition}{PJR \cite{PJR}}
A committee $W$ is said to satisfy \emph{Proportional Justified Representation} if there does not exist a group of voter $V' \subseteq V$ with size $|V'| \geq l\frac{n}{k}$ for $l \in \{1, 2, \dots k\}$ such that $|\cap_{i \in V'}A_i| \geq l$ but 
$|(\cup_{i \in V'}A_i) \cap W| < l$.
\end{definition}
The idea behind \emph{JR} and \emph{PJR} is that if voters in large enough groups are inclined to have similar choices, then at least some voters of the group should get some representation in the committee $W$. 
In this paper, we generalize dichotomous preferences to trichotomous preferences which allows an extension in expressiveness to the voters by allowing them not only to elicit approval or disapproval but also indifference over the candidates in the candidate set. We represent the position of a candidate $c$ for a voter $i$ such that $pos_c(i) \in \{1, 0, -1\}$ if the candidate lies in the approval, indifference and disapproval set respectively of voter $i$. We define the positional score of a candidate $c$ as the sum of positions of the candidate in the preference ballots of all voters in the electorate i.e. $\Sigma_{i \in V}pos_c(i)$. Moreover, we use $[k]$ as an abbreviation for the set $\{1, 2, \dots k\}$.  
\begin{remark}\label{remark:remark1}
A dichotomous approval voter profile \textbf{$A_{dic}$} = $(A_1, A_2, \dots A_n)$ is essentially a trichotomous voter profile \textbf{$A_{tri}$} = ~$((A_1^+, A_1^-), \dots (A_n^+, A_n^-))$ with $A_i^+ \cup A_i^- = C \text{ } \forall i \in V$, or $A_i^0 = \emptyset$ $\forall i \in V$ which means that a trichotomous profile with every voter casting an empty indifference ballot is essentially a dichotomous profile. 
\end{remark}


==> Voting with Negative Feelings/ConditionalProof.tex <==
\begin{prop}
WTPSC implies Generalized Proportional Solid Coalition. 
\end{prop}
\begin{proof}
Let us assume that the committee $W$ satisfies WTPSC, which means that for all `large enough' trichotomous Solid Coalitions, there is a proportional representation in the committee. We take into account the following three cases where the set of voters which forms a solid coalition is large enough i.e. $V' \geq l\frac{n}{k}$ and the nature of the set of candidates over which the voters form the solid coalition varies.
\begin{itemize}
    \item If a set of voters $V'$ form a trichotomous solid coalition for a set of candidates $C' = C$, then every committee trivially satisfies Hare-PSC since there always exists a subset $C''$ large enough in the committee such that the candidates in it are preferred at least as much as the least preferred candidates by some voter in the solid coalition.
    \item Assume that $\forall i \in V'$ and $\forall c' \in C'$, \rutvik{to check notations in handbook of COMSOC} $c' \in max_i(V')$.\footnote{\noindent$max_i(C)$ returns the most preferred candidates from C with respect to the weak ranking of the $i^{th} $voter} So, $C' \subseteq (\cup_{i \in V'} A_i^+ \setminus \cup_{i \in V'} A_i^-)$. Since the committee satisfies WTPSC, $(\cup_{i \in V'}A_i^+) \cap W \geq l$ and since every candidate in the set $C'$ belongs to $A_i^+$ for all $i \in V'$ there always exists a subset of candidates $C'' \subseteq W$ of size $min(|C'|, l)$ such that  $\forall c'' \in C''$
    $$\exists i \in V': c'' \succeq c^{(i, |C'|)}$$
    \item Now assume that $\forall i \in V'$ and $\forall c' \in C'$, $c' \in max_{\succ_i}(C)$ or $c' \in indif_{\succ_i}(C)$\footnote{We assume that the set of solidly supported candidates does not contain those candidates which lie in the indifference class of all the voters that form the solid coalition.  } Since this set of voters does form a solid coalition, $\forall c' \in C' \text{, } \exists i \in V'\text{such that } \\
    c' \in A_i^+$\footnote{refer footnote 2}. Since every candidate in $C'$ belongs to the approval class of at least one of the voters in the solid coalition, $C' \subseteq \cup_{i \in V'}A_i+ \setminus \cup_{i \in V'}A_i^-$. Again since the committee satisfies WTPSC and additionally every candidate in $C'$ belongs to $A_i^+$ for some voter $i \in V'$, there always exists a subset of candidates $C'' \subseteq W$ of size $min(|C'|, l)$ such that $\forall c'' \in C''$ 
    $$\exists i \in V' : c'' \succeq c^{(i, |C'|)}$$
    
\end{itemize}
The only difference between the second and the third point is that in the second case, the \emph{solidly supported candidates} lie in the approval sets of each and every voter, while in the latter case, they either lie in the approval set of at least one voter. 
\end{proof}




\begin{itemize}

\item 
It makes sense to consider single-winner elections, multiwinner elections, and participatory budgeting.

\item
One thing that we can say is that adding the possibility of expressing negative feelings is, informally speaking, more ``expressive''.

To make this informal claim of some weight, we can consider the example of a voter which is OK with all the alternatives beside one; without negative feelings, he can give the cumulative vote $[1/m, \ldots, 1/m, 0]$, but the difference between $1/m$ and $0$ is very small. However, with the possibility of expressing negative feelings, such a voter can say $[0, \ldots, 0, -1]$, which is much more intense and closer to what the voter wants to express.

\item Suppose we now consider that the set of voters 
Hopefully we can show some impossibility results and, thus, formally demonstrate that there are some things that cannot be achieved without adding the possibility of expressing negative feelings.


\item
Say something about ``chores''.

\item
Some related work: ``Dilemma with approval and disapproval votes'' (and other stuff from Annick).

\end{itemize}


\nimrod{and here our paper ends, yes?}

\section{Ordinal Voting with Negative Feelings}

A natural way of adding negative feelings to ordinal elections would be to let each voter specify a ranking \textbf{and} a number between $0$ and $|A| + 1$, understood as the ``cutting point'' in the ordinal ranking, specifically such that alternatives to the left of the cutting point are to be understood as making positive feelings while alternatives to the right of the cutting point are to be understood as making negative feelings.

E.g., a vote over $A = \{a, b, c\}$ could be $a > b\ |\ c$, where $|$ means the cutting point. Then, such a vote is understood that $a$ is the best choice, then $b$, and then $c$ makes me feel negative. \\



\section{Cumulative voting with negative feelings}

A natural way of adding negative feelings to cumulative elections would be to let each voter specify a ``division of one coin'' between the alternatives \textbf{and} labeling each item with either ``positive'' or ``negative''.

Pictorially, this is like dot-voting, but where participants do not simply get stickers, but get Reversi disks.

\nimrod{Perhaps actually this is the most interesting thing that we can offer..}

\nimrod{Motivation also from the bench example}


\subsection{Single-Winner Reversi Voting}

So each voter gets $t$ Reversi disks which she can place on each of the alternatives, either as positive (say, green) or negative (say, red). Then, the \emph{score} of each alternative equals the number of green disks on it minus the number of red disks on it, and an alternative with the highest score wins.


\subsection{Multiwinner Reversi Voting}

We can use Reversi voting also for multiwinner voting by considering a $k$-best version of it:
  The \emph{score} of each alternative equals the number of green disks on it minus the number of red disks on it, and we select the $k$ top alternatives when sorted in decreasing order of their score.


\subsection{Reversi Voting for Participatory Budgeting}

We can adapt our CSTV to use Reversi voting. To see why it is important, consider the following example:
  With our CSTV we can run into the problem as follows.
  There are $3$ items, $a$, $b$, and $c$. There is budget limit $2$, and all items cost the same, that is $1$ (unit cost; so this is actually multiwinner election).
  Now, there are $5$ voters.
  For the story, say that voter $v_4$ and $v_5$ already voted, as follows:
  $v_4 : 0, 0, 1$,
  $v_5 : 0, 0, 1$.
  So, $c$ gets two points (size of stash), and $a$ and $b$ get zero.
  For the story, say that $v_1, v_2, v_3$ have very strong negative feelings towards $c$.
  Now, if we do our normal CSTV, then, even though $\{v_1, v_2, v_3\}$ is a voter majority, they cannot make it so as to not fund $c$.

However, if we use negative feelings (i.e., adapt Reversi voting here), then $v_1, v_2, v_3$ can vote as follows:
  $v_1 : 1/6, 1/6, -2/3$,
  $v_2 : 1/6, 1/6, -2/3$,
  and
  $v_3 : 1/6, 1/6, -2/3$
and get $c$ not to be funded.

==> Voting with Negative Feelings/diagram.tex <==
\begin{figure}
    \centering
    \includegraphics[scale = 0.9]{IMAGE.jpg}
    \caption{Relationship between the proposed Class I and Class II axioms}
    \label{fig:my_label}
\end{figure}
